System- and Software-level Architecting Harmonization Practices for Systems-of-Systems -- An exploratory case study on a long-running large-scale scientific instrument

The problems caused by the gap between system- and software-level architecting practices, especially in the context of Systems of Systems where the two disciplines inexorably meet, is a well known issue with a disappointingly low amount of works in the literature dedicated to it. At the same time, organizations working on Systems of Systems have been developing solutions for closing this gap for many years now. This work aims to extract such knowledge from practitioners by studying the case of a large-scale scientific instrument, a geographically distributed radio telescope to be more specific, developed as a sequence of projects during the last two decades. As the means for collecting data for this study we combine online interviews with a virtual focus group of practitioners from the organization responsible for building the instrument. Through this process, we identify persisting problems and the best practices that have been developed to deal with them, together with the perceived benefits and drawbacks of applying the latter in practice. Some of our major findings include the need to avoid over-reliance on the flexibility of software to compensate for incomplete requirements, hidden assumptions, as well as late involvement of system architecting, and to facilitate the cooperation between the involved disciplines through dedicated architecting roles and the adoption of unifying practices and standards.

==> research_design.tex <==


Three research questions:

This is an exploratory  case study in the domain of scientific SoS architecting, we proposed three research questions:

Interdisciplinary problems posed in the interplay between systems engineering-related disciplines and software engineering.

Practices developed or adapted to harmonize the interplay between these disciplines

Benefits/drawbacks from said practices

Collected data: 

two steps - interview to 5 subjects - semi structured format. We asked about both projects

focus group with X subjects: amplify and complete the findings from the interviews, as well explore: benefits and drawbacks. THUS discussion points will be derived from the analysis of the interviews.


How structured discussions should be?

VFG using asynchronous, text-based CMC... all the communications of the group can be saved and reflected on at any time.

Researched will act as a moderator, by starting the discussion threads. The participants will respond on their own convenience, within an stipulated deadline





